Counting in Practical Anonymous Dynamic Networks is Polynomial

Anonymous Dynamic Networks is a harsh computational environment due to changing topology and lack of identifiers. Computing the size of the network, a problem known as Counting, is particularly challenging because messages received cannot be tagged to a specific sender. Previous works on Counting in Anonymous Dynamic Networks do not provide enough guarantees to be used in practice. Indeed, they either compute only an upper bound on the network size that may be as bad as exponential, or guarantee only double-exponential running time, or do not terminate, or guarantee only eventual termination without running-time guarantees. Faster experimental protocols do not guarantee the correct count. Recently, we presented the first Counting protocol that computes the exact count with exponential running-time guarantees. The protocol requires the presence of one leader node and knowledge of any upper bound Delta on the maximum number of neighbors that any node will ever have. In the present work, we complement the latter theoretical study evaluating the performance of such protocol in practice. We tested a variety of network topologies that may appear in practice, including extremal cases such as trees, paths, and continuously changing topologies. We also tested networks that temporarily are not connected. Our simulations showed that the protocol is polynomial for all the inputs tested, paving the way to use it in practical applications where topology changes are predictable. The simulations also provided insight on the impact of topology changes on information dissemination. To the best of our knowledge, this is the first experimental study that shows the possibility of computing the exact count in polynomial time in a variety of Anonymous Dynamic Networks that are worse than expected in practice.

==> analysis.tex <==
%!TEX root = draft.tex

\section{Analysis}
\label{sec:analysis}

The following notation will be used. The energy of node $i$ at the beginning of round $r$, is denoted as $e_i^r$, which is also generalized to any set of nodes $S\subseteq V$ as $e_S^r=\sum_{i\in S}e_i^r$. 
For any given round $r$ and node $i$, 
%let the degree of $i$ be $d_i^r$ and the average energy of $i$'s neighbors be $\overline{e}_{N_i}^r$. 
let the set of neighbors of $i$ be $N_i^r$ and the average energy of $i$'s neighbors be $\overline{e}_{N_i^r}$. 
The superindex indicating the round number will be omitted when clear from context or irrelevant.
Also, at any time, let $\sum_{i\in V} e_i$ be called the \emph{system energy} and $\sum_{i\in V\setminus\{\ell\}} e_i$ be called the \emph{energy left}. 
At the beginning of each iteration of the protocol, that is, for each new size estimate $k$, the energy of the leader is reset to zero and the energy of the non-leader nodes is reset to $1$. Thus, the system energy is $\sum_{i\in V} e_i=n-1$ and the energy left is $\sum_{i\in V\setminus\{\ell\}} e_i=n-1$.

%The following lemmata show the correctness of each phase of the Counting Protocol (Algorithms~\ref{algo:leader} and~\ref{algo:no-leader}). 
%
%\begin{lemma}
%\label{lemma:collect}
%{\bf Correctness of the Collection Phase:}
%For any network of $n$ nodes, including a leader $\ell$, running the Counting Protocol the following holds.
%For any estimate of the size of the network $k\leq n$ and constant $c>1$, 
%there exists a function $\tau(k)>0$ such that, 
%if $k=n$ and the Collection Phase is executed for at least $\tau(k)$ rounds, then at the end of the phase the leader has energy $e_\ell\geq k-1-1/k^c$.
%\end{lemma}
%\begin{proof}
%In order to prove the claim, it is enough to show that as long as there is energy left, the leader will eventually receive more energy.
%Given that $k\leq n$, the system energy is $n-1\geq k-1$. Thus, while $e_\ell<k-1-1/k^c$, there is energy left.
%For the sake of contradiction, assume that at the beginning of some round $r$ the energy left is some $\varepsilon>0$, but the leader does not increase its energy in any round $r'>r$.
%Consider the partition of nodes $\{V_1^r,V_2^r\}$ defined by the non-leader nodes whose energy is positive at the beginning of round $r$. That is, $\forall i\in V_1^r: e_i^r>0$, $\ell\in V_2^r$, and $\forall i\in V_2^r\setminus\{\ell\}: e_i^r=0$. $V_1^r$ is not empty since the energy left is positive. By 1-interval connectivity, there must exist a link $u,v$, such that $u\in V_1^r$ and $v\in V_2^r$. If $v=\ell$, due to the energy transfer in Line~\ref{transferleader} in Algorithm~\ref{algo:leader}, the leader increases its energy in round $r$, which is a contradiction. If on the other hand it is $v\neq\ell$, due to the energy transfer in Line~\ref{transfernonleader} in Algorithm~\ref{algo:no-leader}, $v$ increases its energy in round $r$. Thus, at the beginning of round $r+1$ we have $|V_1^{r+1}|\geq|V_1^r|+1$ and $|V_2^{r+1}|\leq|V_2^r|-1$. It can be seen inductively that after enough number of rounds the leader will increase its energy which is a contradiction. Hence, the claim follows.
%\qed
%\end{proof}
%
%The following lemmas will be needed.

\begin{lemma}
\label{lemma:nodeenergy}
For any network of $n$ nodes, including a leader $\ell$, running the Counting Protocol under the communication and connectivity models defined the following holds.
For any given node $i\in V\setminus\{\ell\}$ and for any given round $r$ of the Collection Phase, it is $e_i^r\leq 1$.
\end{lemma}
\begin{proof}
Fix some arbitrary (non-leader) node $i$. 
Consider the transition between round $r$ and $r+1$. 
We have that
$$e_i^{r+1} \leq e_i^r + \overline{e}_{N_i^r} \frac{|N_i^r|}{2\Delta} - e_i^r \frac{|N_i^r|}{2\Delta} = e_i^r + (\overline{e}_{N_i^r} - e_i^r) \frac{|N_i^r|}{2\Delta}.$$

If $\overline{e}_{N_i^r} \leq e_i^r$, then $e_i^{r+1} \leq e_i^r$. 
That is, $i$'s energy does not increase from round $r$ to round $r+1$.
If on the other hand it is $\overline{e}_{N_i^r} > e_i^r$, we have
$$e_i^{r+1} \leq e_i^r + (\overline{e}_{N_i^r} - e_i^r)/2 = (e_i^r + \overline{e}_{N_i^r})/2.$$

That is, the energy of $i$ in round $r+1$ is at most the average between the energy of $i$ in round $r$ and the average of $i$'s neighbors' energy in round $r$. 

Now consider the evolution of the protocol along many rounds.
We ignore the rounds when $\overline{e}_{N_i^r} \leq e_i^r$ since they do not increase the energy. 
For the other rounds, given that all nodes start with energy $1$, and that the average of some numbers cannot be bigger than the maximum, the energy at any given node cannot get bigger than $1$. Hence, the claim follows. 
%\qed
\end{proof}

\begin{lemma}
\label{lemma:broadcast}
For any network of $n$ nodes, under the communication and connectivity models defined, the following holds.
If a message $m$ is held by all nodes in a set $V_1\subseteq V$, after $|V|-|V_1|$ rounds when every node holding the message broadcasts $m$ in each round, all nodes in $V$ hold the message.
\end{lemma}
\begin{proof}
For any round $r>0$, consider the partition of nodes $\{V_1^r,V_2^r\}$ defined by the nodes holding the message at the beginning of round $r$. That is, $\forall i\in V_1^r$ the node $i$ holds $m$ and $\forall j\in V_2^r$ the node $j$ does not hold $m$. 
By 1-interval connectivity, there must exist a link $u,v$, such that $u\in V_1^r$ and $v\in V_2^r$. Given that all nodes holding the message broadcast $m$, $v$ must receive the message in round $r$. 
Thus, at the beginning of round $r+1$ it is $|V_1^{r+1}|\geq|V_1^r|+1$ and $|V_2^{r+1}|\leq|V_2^r|-1$. Applying the same argument inductively, after $|V_2^{r+1}|$ more rounds all nodes hold the message.
\end{proof}

The following lemma is a straightforward application of Lemma~\ref{lemma:broadcast} to the Notification Phase, where the message broadcasted is $\langle Halt\rangle$ for the first time when $k=n$.

\begin{lemma}
\label{lemma:halt}
{\bf Correctness of the Notification Phase:}
For any network of $n$ nodes, including a leader $\ell$, running the Counting Protocol under the communication and connectivity models defined the following holds.
If at the end of the Verification Phase $IsCorrect=true$, then at the end of the Notification Phase all nodes stop the Counting Protocol holding the size $n$.
\end{lemma}

\begin{lemma}
\label{lemma:correctness}
{\bf Correctness of the Verification Phase:}
For any network of $n>3$ nodes, including a leader $\ell$, running the Counting Protocol under the communication and connectivity models defined the following holds.
%For any estimate of the size of the network $k$ and constant $c>1$, if at the end of the Collection Phase it is $e_\ell\geq k-1-1/k^c$, then at the end of the Verification Phase $IsCorrect=true$ if and only if $k=n$.
For any estimate of the size of the network $k$ and constant $c>1$, at the end of the Verification Phase $IsCorrect=true$ if and only if $k=n$.
\end{lemma}
\begin{proof}
We start observing that, for each estimate $k$, each non-leader node is initialized with one unit of energy (Line~\ref{initone} in Algorithm~\ref{algo:no-leader}) and the leader's energy is initialized to $0$ (Line~\ref{initzero} in Algorithm~\ref{algo:leader}). Until a new iteration of the outer loop (in both algorithms) is executed, no energy is lost or gained by the system as a whole. Hence, the system energy is always $n-1$.

%We prove first that, if $k=n$, at the end of the Verification Phase it is $IsCorrect=true$.
%Given that $k=n$, the system energy is $k-1$. Thus, it must be $e_\ell\leq k-1$ and $IsCorrect$ is not set to false in Line~\ref{false2} of Algorithm~\ref{algo:leader}.
%Given the assumption that $e_\ell\geq k-1-1/k^c$ at the end of the Collection Phase,
%we know that the energy left at the beginning of the Verification Phase is 
%$e_{V\setminus \{\ell\}} = k-1-e_\ell \leq 1/k^c$.
%Therefore, no non-leader node could have more than that energy. 
%That is, $\forall i\in V\setminus \{\ell\} : e_i\leq 1/k^c$. Thus, during the Verification Phase, the leader will not be able to detect a node with energy bigger than $1/k^c$.
%Therefore, $IsCorrect$ is not set to false in Line~\ref{false1} of Algorithm~\ref{algo:leader} either.
%There is no other line where $IsCorrect$ is set to false. Hence, at the end of the Verification Phase it is $IsCorrect=true$.
We prove first that, if $k=n$, at the end of the Verification Phase it is $IsCorrect=true$.
Given that $k=n$, the system energy is $k-1$ and therefore $e_\ell\leq k-1$. Also because $k=n$, we know that after the Collection Phase it is $e_\ell\geq k-1-1/k^c$ by definition of $\tau(k)$.
Therefore, $IsCorrect$ is not set to false in Line~\ref{false2} of Algorithm~\ref{algo:leader}.
Also because $e_\ell\geq k-1-1/k^c$ at the end of the Collection Phase,
we know that the energy left at the beginning of the Verification Phase is 
$e_{V\setminus \{\ell\}} = k-1-e_\ell \leq 1/k^c$.
Therefore, no non-leader node could have more than that energy. 
That is, $\forall i\in V\setminus \{\ell\} : e_i\leq 1/k^c$. Thus, during the Verification Phase, the leader will not be able to detect a node with energy bigger than $1/k^c$.
Therefore, $IsCorrect$ is not set to false in Line~\ref{false1} of Algorithm~\ref{algo:leader} either.
There is no other line where $IsCorrect$ is set to false. Hence, at the end of the Verification Phase it is $IsCorrect=true$.

We prove now the other direction of the implication. That is, if at the end of the Verification Phase $IsCorrect=true$, then it is $k=n$.
For the sake of contradiction, assume that $IsCorrect=true$ but $k\neq n$.
Notice that $k$ cannot be larger than $n$, because the estimate is increased one by one, we already proved that if $k=n$ at the end of the Verification Phase it is $IsCorrect=true$, and Lemma~\ref{lemma:halt} shows that all nodes would have stopped running the protocol.
Thus, we are left with the case when $k<n$.

Notice that if $e_\ell > k-1$ the variable $IsCorrect$ is set to false in Line~\ref{false2} of Algorithm~\ref{algo:leader}.
Hence, it must be $e_\ell \leq k-1$ and,
given that the system energy is $n-1$, the energy left is $e_{V\setminus \{\ell\}}\geq n-k$.
This energy left is stored in the $n-1$ non-leader nodes. 
Hence, there must exist some node $j\in V\setminus\{\ell\}$ in the network such that $e_j\geq (n-k)/(n-1)$.
If $IsCorrect=true$ it means that the leader did not detect a node with energy bigger than $1/k^c$ in Line~\ref{detect} of Algorithm~\ref{algo:leader}. 
However, for any $2\leq k\leq n-1$, $n>3$, and $c>1$, it is $1/k^c<(n-k)/(n-1)$ which means that such node must exist. 

To see why the latter inequality is true, we verify that $k^c(n-k)-n+1>0$ as follows. With respect to $k$, this function has a maximum for $k=cn/(c+1)$. 
That is, for $2\leq k\leq n-1$ (recall that we are in the case $k<n$), the function has minima in $2$ and $n-1$. 
Then, it is enough to verify that $2^c(n-2)-n+1>0$, which is true for any $c>1$ and $n>3$, 
and that $(n-1)^c-n+1>0$, which is also true for any $c>1$ and $n\geq 2$.

Thus, to complete the proof, it is enough to show that $1+k^{c+1}/(k^c-1)$ rounds are enough to detect a node with energy bigger than $1/k^c$.
To do that, we upper bound the number of nodes in the network with energy at most $1/k^c$ as follows. We know that at any time when the leader has energy $e_\ell$, the energy left is $n-1-e_\ell$. Let $S\subseteq V$ be the set of nodes with energy at most $1/k^c$. Then, we have that $n-1-e_\ell=\sum_{j\in S}e_j+\sum_{k\in V\setminus S}e_k$. To maximize the size of $S$, we minimize the size of $V\setminus S$ assuming that all nodes in $V\setminus S$ have maximum energy, which according to Lemma~\ref{lemma:nodeenergy} is at most 1. Then, we have that $n-1-e_\ell=\sum_{j\in S}e_j+(n-|S|)$ which yields $|S|-1-e_\ell=\sum_{j\in S}e_j$ Given that $\sum_{j\in S}e_j\leq |S|/k^c$, we have that
%$|S|-1-e_\ell\leq |S|/k^c$
%$|S|-|S|/k^c\leq 1+e_\ell$
%$|S|(1-1/k^c)\leq 1+e_\ell$
$|S|\leq (1+e_\ell)/(1-1/k^c)$.
%
Recall that $e_\ell \leq k-1$ because $IsCorrect$ would have been set to false in Line~\ref{false2} of Algorithm~\ref{algo:leader} otherwise.
Replacing, we get $|S|\leq k^{c+1}/(k^c-1)$. 

Let $\{V_1,V_2\}$ be a partition of $V$ such that $V_2=S\cup\{\ell\}$. Recall that, for any $v\in V_1$ it is $e_v>1/k^c$. 
Using Lemma~\ref{lemma:broadcast}, we know that 
$|V_2|=1+k^{c+1}/(k^c-1)$ iterations in the Verification Phase of Algorithm~\ref{algo:leader} are enough for the leader to detect that there is a node with energy larger than $1/k^c$, which contradicts our assumption that $IsCorrect=true$. 
%\qed
\end{proof}

The following theorem establishes our main result. 

\begin{theorem}
\label{thm:all}
For any anonymous dynamic network of $n>3$ nodes, including a leader $\ell$, and for any constant $c>\log 5$, the following holds.
If the adversarial topology is limited by a maximum degree $\Delta$ and the connectivity model defined, and nodes run the Counting Protocol in Algorithms~\ref{algo:leader} and~\ref{algo:no-leader} under the communication model defined, after $r$ rounds, all nodes stop holding the size of the network $n$, where
\begin{align*}
r 
&< n(n+3)+\ln n-4+\sum_{k=2}^n \tau(k).
\end{align*}
Where $\tau(k)$ is a function such that, if $k=n$ and the Collection Phase is executed for at least $\tau(k)$ rounds, then at the end of the phase the leader has energy $e_\ell\geq k-1-1/k^c$.
\end{theorem}
\begin{proof}
Correctness is a direct consequence of Lemmas~\ref{lemma:halt} and~\ref{lemma:correctness}. 
The running time is obtained adding the number of iterations of each phase, as follows.
\begin{align*}
r 
&= \sum_{k=2}^n \left(\tau(k)+\left\lceil1+\frac{k}{1-1/k^c}\right\rceil+k\right)\\
&\leq \sum_{k=2}^n \left(\tau(k)+2+\frac{k}{1-1/k^c}+k\right)\\
%&= 2n-2+\sum_{k=2}^n \left(\tau(k)+\frac{k}{1-1/k^c}+k\right)\\
%&= 2n-2+\sum_{k=2}^n \left(\tau(k)+\frac{k^{1+c}}{k^c-1}+k\right)\\
%&= 2n-2+\sum_{k=2}^n \left(\tau(k)+\frac{2k^{1+c}-k}{k^c-1}\right)\\
%&= 2n-2+\sum_{k=2}^n \left(\tau(k)+k\frac{2k^{c}-1}{k^c-1}\right)\\
%&= 2n-2+\sum_{k=2}^n \left(\tau(k)+k\left(2+\frac{1}{k^c-1}\right)\right)\\
%&= 2n-2+2(n(n+1)/2-1)+\sum_{k=2}^n \left(\tau(k)+\frac{k}{k^c-1}\right)\\
%&= 2n-2+n(n+1)-2+\sum_{k=2}^n \left(\tau(k)+\frac{k}{k^c-1}\right)\\
%&= 2n+n(n+1)-4+\sum_{k=2}^n \left(\tau(k)+\frac{k}{k^c-1}\right)\\
&= n(n+3)-4+\sum_{k=2}^n \left(\tau(k)+\frac{k}{k^c-1}\right).
\end{align*}

Using that $k/(k^c-1)<1/k$ for any $c>\log 5$ and $k\geq 2$, we obtain the following. 
\begin{align*}
r 
&< n(n+3)-4+\sum_{k=2}^n \left(\tau(k)+\frac{1}{k}\right)\\
&\leq n(n+3)+\ln n-4+\sum_{k=2}^n \tau(k).
\end{align*}
%\qed
\end{proof}

Bounding the running time of the Collection Phase using Lemma 2 in~\cite{conscious} in Theorem~\ref{thm:all}, the following corollary is obtained.

\begin{corollary}
\label{cor:exp}
For any anonymous dynamic network of $n>6$ nodes, including a leader $\ell$, the following holds.
If the adversarial topology is limited by a maximum degree $1\leq\Delta\leq n-1$ and the connectivity model defined, and nodes run the Counting Protocol in Algorithms~\ref{algo:leader} and~\ref{algo:no-leader} under the communication model defined, after $r$ rounds, all nodes stop holding the size of the network $n$, where
\begin{align*}
r 
&< \frac{(2\Delta)^{n+1}(n+1)\ln (n+1)}{\ln(2\Delta)}.
\end{align*}
\end{corollary}
\begin{proof}
Lemma 2 in~\cite{conscious} proves that, for any estimate $k\geq n$ and integer $\rho>0$, starting with $e_\ell=0$ and $e_i=1$ for all $i\in V\setminus \{\ell\}$, after running $\rho k$ rounds of the energy transfer protocol the energy stored in the leader is $e_\ell \geq n(1-(((2\Delta)^{k}-1)/(2\Delta)^{k})^\rho)$. 
Notice in Theorem~\ref{thm:all} that the condition $e_\ell\geq k-1-1/k^c$ only applies when $k=n$.
Thus, it is enough to find $\rho$ such that 
\begin{align*}
k\left(1-\left(\frac{(2\Delta)^{k}-1}{(2\Delta)^{k}}\right)^{\rho}\right) &\geq k-1-1/k^c\\
%k-k\left(\frac{(2\Delta)^{k}-1}{(2\Delta)^{k}}\right)^{\rho} &\geq k-1-1/k^c\\
%k\left(\frac{(2\Delta)^{k}-1}{(2\Delta)^{k}}\right)^{\rho} &\leq 1+1/k^c\\
%\left(\frac{(2\Delta)^{k}-1}{(2\Delta)^{k}}\right)^{\rho} &\leq \frac{1+1/k^c}{k}\\
%\left(\frac{(2\Delta)^{k}}{(2\Delta)^{k}-1}\right)^{\rho} &\geq \frac{k}{1+1/k^c}\\
%\left(\frac{1}{1-1/(2\Delta)^{k}}\right)^{\rho} &\geq \frac{k}{1+1/k^c}\\
\rho &\geq \frac{\ln (k/(1+1/k^c))}{\ln\left(1/(1-1/(2\Delta)^{k})\right)}.
\end{align*}

Using that $1-x\leq e^{-x}$ for $x\leq 1$, it is enough to have $\rho = \lceil(2\Delta)^k \ln k\rceil$. Replacing in Theorem~\ref{thm:all}, we obtain

\begin{align*}
r 
&< n(n+3)+\ln n-4+\sum_{k=2}^n k\lceil(2\Delta)^k \ln k\rceil\\
&\leq n(n+3)+\ln n-4+\sum_{k=2}^n k(1+(2\Delta)^k \ln k)\\
%&= n(n+3)+\ln n-4+(n(n+1)/2)-1+\sum_{k=2}^n k(2\Delta)^k \ln k\\
%&= n(n+3)+(n(n+1)/2)+\ln n-5+\sum_{k=2}^n k(2\Delta)^k \ln k\\
%&= n(n+3+(n+1)/2)+\ln n-5+\sum_{k=2}^n k(2\Delta)^k \ln k\\
&= n(3n+7)/2+\ln n-5+\sum_{k=2}^n k(2\Delta)^k \ln k.
\end{align*}
 
Bounding with the integral,
\begin{align*}
r &< n(3n+7)/2+\ln n-5+\int_{k=2}^{n+1} k(2\Delta)^k \ln k~\mathrm{d} k\\
&= n(3n+7)/2+\ln n-5+\frac{(2\Delta)^k((k\ln(2\Delta)-1)\ln k-1)+\textrm{Ei}(k\ln(2\Delta))}{\ln^2(2\Delta)}\bigg|_2^{n+1}\\
&\leq n(3n+7)/2+\ln n+\frac{(2\Delta)^{n+1}(((n+1)\ln(2\Delta)-1)\ln (n+1)-1)+\textrm{Ei}((n+1)\ln(2\Delta))}{\ln^2(2\Delta)}.
\end{align*}

%Using that $(2\Delta)^x\geq \textrm{Ei}(x\ln(2\Delta))$ for any $1\leq \Delta\leq x-2$ and $x\geq 2$, \textcolor{red}{checked with mathematica only, prove it.}

Using that $\textrm{Ei}(\ln x)=\textrm{li}(x)< x$, for any real number $x\neq 1$,
it is $\textrm{Ei}((n+1)\ln (2\Delta))<(2\Delta)^{n+1}$. Replacing,
%WIKIPEDIA:https://en.wikipedia.org/wiki/Logarithmic_integral_function

\begin{align*}
r &< n(3n+7)/2+\ln n+\frac{(2\Delta)^{n+1}((n+1)\ln(2\Delta)-1)\ln (n+1)}{\ln^2(2\Delta)}\\
&= n(3n+7)/2+\ln n
+\frac{(2\Delta)^{n+1}(n+1)\ln (n+1)}{\ln(2\Delta)}
-\frac{(2\Delta)^{n+1}\ln (n+1)}{\ln^2(2\Delta)}.
\end{align*}
Using that $n(3n+7)/2+\ln n<(2\Delta)^{n+1}\ln (n+1)/\ln^2(2\Delta)$ for any $n>6$ and $1\leq\Delta\leq n-1$, the claim follows.
%
%The latter inequality can be proved as follows.
%We show first that
%\begin{align*}
%\ln^2(2\Delta)n(3n+7) &< (2\Delta)^{n+1}\ln (n+1)\\
%\ln\ln^2(2\Delta)+\ln(n(3n+7)) &< (n+1)\ln(2\Delta)+\ln\ln (n+1)\\
%2\ln\ln(2\Delta)+\ln(n(3n+7)) &< n\ln(2\Delta)+\ln(2\Delta)+\ln\ln (n+1)\\
%\end{align*}
%Which is true because $2\ln\ln(2\Delta)<\ln(2\Delta)$ and $\ln(n(3n+7))<n\ln(2\Delta)+\ln\ln (n+1)$ for any $n>6$ replacing $\Delta$ by its lower and upper bounds.
%And finally that
%\begin{align*}
%2\ln^2(2\Delta)\ln n &< (2\Delta)^{n+1}\ln (n+1)
%\end{align*}
%Which is true for any $n\geq 1$ replacing $\Delta$ by its lower and upper bounds.
%\qed
\end{proof}

%\textcolor{red}{THE FOLLOWING SEEMS TO BE FALSE}
%
%The latter corollary uses an exponential upper bound on the cost of the Collection Phase. A natural question is whether a better upper bound can be proved. The following theorem answers such question negatively for \emph{gossip-based} protocols (also called \emph{mass-distribution}, \emph{energy transfer}, etc.~\cite{KDGgossip,flowupdate,FMT:aggJournal,conscious}). That is, any protocol where each node holds a value (mass, energy, input variable, etc.) and repeatedly transfers a fraction of such value to neighbors.
%The theorem is presented for synchronous even transfer. The same claim can be proved for asynchronous uneven transfer with a more laborious derivation.
%
%\begin{theorem}
%\label{thm:lb}
%For any $n>2$ and $c>0$, there exists a dynamic network such that any gossip-based implementation of the Collection Phase, where energy is shared evenly among neighbors and the transfer is carried synchronously in rounds, requires exponential number of rounds to collect more than $n-1-1/n^c$ energy at the leader node. 
%\end{theorem}
%
%\begin{proof}
%Consider a network where all nodes are located in a single path ending at the leader node.
%For reference, let us label the nodes as $0,1,2,\dots,n-1$, where node $0$ is the leader, and let the rounds of energy transfer be numbered as $1,2,\dots$. Recall that $e_i^r$ is the energy of node $i$ at the beginning of round $r$.
%Initially, the energy at each node is $e_\ell^1=0$ and $e_i^1=1$, for $0<i<n$.
%That is, initially the total energy in the network is $n-1$, and given that no energy is lost or gained, the total energy throughout all the execution of the Collection Phase stays the same. 
%Also notice that, while executing the Collection Phase, the energy in non-leader nodes is monotonically non-increasing towards the leader. 
%That is, for any round $r\geq1$ and pair of nodes $j,k$, such that $0<j<k\leq n-1$, it is $e_{j}^{r}\leq e_{k}^{r}$. 
%
%For any given execution of a gossip-based implementation of the Collection Phase, consider the first round $r$ when $e_\ell^r\geq n-1-1/n^c$. 
%In round $r$, the total energy in non-leader nodes is at most $1/n^c$, hence we know that for any node $i>0$ it is $e_{i}^r\leq 1/n^c$.
%We compute now a lower bound on the minimum number of rounds needed for all non-leader nodes  to reach an energy value at most $1/n^c$. 
%%
%
%First, we identify what is the energy distribution that maximizes the energy transferred towards the leader as follows.
%For any given round $r'\leq r$, the amount of energy transferred from node $i$ to node $i-1$, where $1<i\leq n-1$, is maximized when the difference $e_{i}^{r'}-e_{i-1}^{r'}$ is maximized. Thus, we want to find the distribution of energy over non-leader nodes that maximizes \emph{all} energy differences of consecutive non-leader nodes simultaneously. In other words, we have a multi-objective optimization problem on $n-1$ variables, and we need to find a Pareto optimal solution.
%Given that we have no preference over any particular difference, we use the following scalarization into a single-objective optimization problem.
%Subject to $0\leq e_{1}^{r'}\leq e_{2}^{r'}\leq\dots\leq e_{n-1}^{r'}\leq 1$, minimize 
%\begin{align*}
%\sum_{i=1}^{n-2} (e_{i+1}^{r'}-e_{i}^{r'}-\max\{e_{i+1}^{r'}-e_{i}^{r'}\})
%&= \sum_{i=1}^{n-2} (e_{i+1}^{r'}-e_{i}^{r'}-1)\\
%&= -n+1+\sum_{i=1}^{n-2} (e_{i+1}^{r'}-e_{i}^{r'})\\
%&= -n+1 + e_{n-1}^{r'}-e_{1}^{r'}.
%\end{align*}
%Which is minimized when $e_{n-1}^{r'}-e_{1}^{r'}$ is maximized, independently of the energy of all other non-leader nodes.
%Thus, we assume as a worst case that node $n-1$ has energy $1$ and node $1$ has energy $0$. Given that the energy at other non-leader nodes is irrelevant, we assume that it is initially $0$ for all of them, and we compute the minimum number of rounds needed to reduce the energy in node $n-1$ to $1/n^c$.
%%Although such distribution of energy will not appear during the execution, the number of rounds needed is not less than the number computed in such scenario.
%
%In any given round, node $n-1$ transfers a fraction $p$ of its energy to node $n-2$, and $n-2$ a fraction $p$ of its energy to $n-3$, etc. Thus, in each round the leader receives at most a $p^{n-1}$ fraction of $(n-1)$'s energy. Therefore, $r$ must be at least $(1-1/n^c)/p^{n-1}$ which is an exponential function because $p<1$. Thus, the claim follows.
%\qed
%\end{proof}




==> contributions.tex <==
%!TEX root = draft.tex

\subsection*{Contributions}
\label{sec:results}
In the following we summarize the main contributions of our work.
\begin{itemize}
\item Following-up on the Conscious Counting protocol of~\cite{conscious}, we present an improved Counting protocol for \ADNs that computes the exact number of nodes in less than $(2\Delta)^{n+1}(n+1)\ln(n+1)/\ln(2\Delta)$ communication rounds, where $n$ is the number of nodes and $\Delta$ is any upper bound on the maximum number of neighbors that any node will ever have. Our algorithm tolerates worst-case changes of topology, limited to 1-interval connectivity. The protocol requires the presence of one leader node and knowledge of $\Delta$. 

\item The running time of our protocol entails an exponential speedup over the previous best Counting algorithm in~\cite{conscious}, which was proved to run in $O(e^{(\Delta^{2n})}\Delta^{3n})$ communication rounds, which is double-exponential. 
The speedup attained is mainly due to a carefully chosen energy threshold used to verify candidate sizes that are not bigger than the actual size.  
Our analysis shows the correctness of such verification.

\item The time complexity proved identifies the phase where the leader collects energy from all other nodes as the speedup bottleneck for Counting with gossip-based protocols. Indeed, the exponential cost is due to this collection, whereas all other terms in the time complexity are polynomial. In contrast, in the running time of~\cite{conscious} all terms are exponential or double exponential.

%\item We also prove that any gossip-based implementation of the Collection Phase, where energy is shared evenly among neighbors and the transfer is carried synchronously in rounds, requires exponential number of rounds. This result shows that, if any speedup is possible for Counting, a different algorithmic approach should be followed. \textcolor{red}{NOT PROVED}

%\item We evaluate experimentally our protocol on \ADNs where the topology changes for each communication round. The specific topologies are unlabeled trees rooted at the leader, chosen uniformly at random from the equivalence classes defined by isomorphisms, and afterwards pruned to guarantee the maximum degree. Our simulations show that in practice our protocol is \textcolor{red}{TO BE COMPLETED} We also carry an experimental contrast against previous heuristics.  \textcolor{red}{TO BE DECIDED}

%\item If exponential exploration works: faster estimate exploration.
%
%\textcolor{red}{--- 
%The current proof does not seem to be adaptable because, for $k>n$, it is not true that $1/k^c < (n-k)/(n-1)$ in Lemma 4. Also, we need to know that $k$ is too big.
%What would be the algorithm? k is doubled until what? the first detection? how do we guarantee to detect when $k>n$? could we be within boundaries $k-1-1/k^c\leq e_\ell\leq k-1$ with $k>n$ and not detect? if $e_\ell \geq k-1-1/k^c$ then $k$ cannot be much bigger than $n$, but if  $e_\ell < k-1-1/k^c$ can we still detect? ---}
%
%\textcolor{red}{LATEST NEWS ON THIS: Not sure how to do the above but, anyway, I wonder whether it is worth, because the running time ends up being just the term n+1 of the summation, as shown in the corollary. So, having only a logarithmic number of terms in the summation would not change much the running time. I suggest we include a discussion about this issue in the explanation of the algorithm.
%}

\end{itemize}

==> plots75nodes/plot_160IntGnp.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1342,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1342,1229){\makebox(0,0)[r]{\strut{} 20000}}%
      \put(1342,1754){\makebox(0,0)[r]{\strut{} 40000}}%
      \put(1342,2279){\makebox(0,0)[r]{\strut{} 60000}}%
      \put(1342,2804){\makebox(0,0)[r]{\strut{} 80000}}%
      \put(1342,3329){\makebox(0,0)[r]{\strut{} 100000}}%
      \put(1342,3854){\makebox(0,0)[r]{\strut{} 120000}}%
      \put(1342,4379){\makebox(0,0)[r]{\strut{} 140000}}%
      \put(1474,484){\makebox(0,0){\strut{} 0}}%
      \put(2140,484){\makebox(0,0){\strut{} 10}}%
      \put(2806,484){\makebox(0,0){\strut{} 20}}%
      \put(3472,484){\makebox(0,0){\strut{} 30}}%
      \put(4139,484){\makebox(0,0){\strut{} 40}}%
      \put(4805,484){\makebox(0,0){\strut{} 50}}%
      \put(5471,484){\makebox(0,0){\strut{} 60}}%
      \put(6137,484){\makebox(0,0){\strut{} 70}}%
      \put(6803,484){\makebox(0,0){\strut{} 80}}%
      \put(176,2541){\rotatebox{-270}{\makebox(0,0){\strut{}Communication rounds}}}%
      \put(4138,154){\makebox(0,0){\strut{}Network size}}%
      \put(4138,4709){\makebox(0,0){\strut{}$T=160$, average of 20 runs}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2662,4206){\makebox(0,0)[r]{\strut{}$G(n,0.1)$}}%
      \csname LTb\endcsname%
      \put(2662,3986){\makebox(0,0)[r]{\strut{}$G(n,0.2)$}}%
      \csname LTb\endcsname%
      \put(2662,3766){\makebox(0,0)[r]{\strut{}$G(n,0.3)$}}%
      \csname LTb\endcsname%
      \put(2662,3546){\makebox(0,0)[r]{\strut{}$G(n,0.4)$}}%
      \csname LTb\endcsname%
      \put(2662,3326){\makebox(0,0)[r]{\strut{}$G(n,0.5)$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./plots75nodes/plot_160IntGnp}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots75nodes/plot_80IntGnp.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1342,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1342,1229){\makebox(0,0)[r]{\strut{} 20000}}%
      \put(1342,1754){\makebox(0,0)[r]{\strut{} 40000}}%
      \put(1342,2279){\makebox(0,0)[r]{\strut{} 60000}}%
      \put(1342,2804){\makebox(0,0)[r]{\strut{} 80000}}%
      \put(1342,3329){\makebox(0,0)[r]{\strut{} 100000}}%
      \put(1342,3854){\makebox(0,0)[r]{\strut{} 120000}}%
      \put(1342,4379){\makebox(0,0)[r]{\strut{} 140000}}%
      \put(1474,484){\makebox(0,0){\strut{} 0}}%
      \put(2140,484){\makebox(0,0){\strut{} 10}}%
      \put(2806,484){\makebox(0,0){\strut{} 20}}%
      \put(3472,484){\makebox(0,0){\strut{} 30}}%
      \put(4139,484){\makebox(0,0){\strut{} 40}}%
      \put(4805,484){\makebox(0,0){\strut{} 50}}%
      \put(5471,484){\makebox(0,0){\strut{} 60}}%
      \put(6137,484){\makebox(0,0){\strut{} 70}}%
      \put(6803,484){\makebox(0,0){\strut{} 80}}%
      \put(176,2541){\rotatebox{-270}{\makebox(0,0){\strut{}Communication rounds}}}%
      \put(4138,154){\makebox(0,0){\strut{}Network size}}%
      \put(4138,4709){\makebox(0,0){\strut{}$T=80$, average of 20 runs}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2662,4206){\makebox(0,0)[r]{\strut{}$G(n,0.1)$}}%
      \csname LTb\endcsname%
      \put(2662,3986){\makebox(0,0)[r]{\strut{}$G(n,0.2)$}}%
      \csname LTb\endcsname%
      \put(2662,3766){\makebox(0,0)[r]{\strut{}$G(n,0.3)$}}%
      \csname LTb\endcsname%
      \put(2662,3546){\makebox(0,0)[r]{\strut{}$G(n,0.4)$}}%
      \csname LTb\endcsname%
      \put(2662,3326){\makebox(0,0)[r]{\strut{}$G(n,0.5)$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./plots75nodes/plot_80IntGnp}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> related.tex <==
%!TEX root = draft.tex

\section{Related Work}
\label{sec:related}

The following is an overview of previous work on Counting in \ADNs directly related to this paper. Other related work may be found in a survey on Dynamic Networks and Time-varying Graphs by Casteigts et al.~\cite{arnaudSurvey}, and in the papers cited below. 

Worst-case topology changes in \DNs may be limited assuming that the network is always connected (cf.~\cite{spirakis,KuhnLO2010,OW05, conscious}), or sometimes disconnected but for some limited time (cf.~\cite{geocast,PPC:opportunistic,F:delaytolerant,michail2014causality}).
The \emph{$T$-interval} connectivity model was introduced in~\cite{KuhnLO2010}. 
For $T\geq 1$, a network is said to be $T$-interval connected if for every $T$ consecutive rounds the network topology contains a stable connected subgraph spanning all nodes.
In the same paper, a Counting protocol was presented, but it requires each node to have a unique identifier. In~\cite{KuhnLO2010} it is also proved that, if no restriction on the size of the messages is required, the counting problem can be easily solved in $O(n)$ time when nodes have IDs. In our work, we focus on \emph{Anonymous} \DNs. Understanding if a linear counting algorithm exists also when IDs are not available will help to understand the difficulty introduced by anonymity (if any).

A Counting protocol for \ADNs where an upper bound $\Delta$ on the maximum degree is known was presented in~\cite{spirakis}. The adversarial topology is limited only to 1-interval connectivity, but the algorithm obtains only an upper bound on the size of the network $n$, which in the worst case is exponential, namely $O(\Delta^n)$. 
%With respect to time complexity, in the worst case $O(n)$ synchronous rounds of communication are needed. 
In our work, we aim to obtain an exact count, rather than only an upper bound.

The \emph{Conscious Counting} algorithm presented later in~\cite{conscious} does obtain the exact count for the same network model, but requires knowledge of an initial upper bound $K$ on the size of the network. Conscious Counting would be exponential if such upper bound were tight, since it runs in $O(e^{K^2}K^3)$ communication rounds. However, $K$ is obtained using the algorithm in~\cite{spirakis} mentioned above. Consequently,  in the worst case the overall running time of the Conscious Counting Algorithm is $O(e^{(\Delta^{2n})}\Delta^{3n})$, which is double-exponential. In our work, we obtain the exact count in exponential time. That is, we reduce exponentially the best known upper bound for exact Counting.

\ADNs where an upper bound on the maximum degree is not known where also studied~\cite{conscious,oracle,experimentalConscious}. In~\cite{conscious}, the protocol does not have a termination condition. That is, nodes running the protocol do not know whether the correct count has been reached or not. Hence, they have to continue running the protocol forever. In a companion paper~\cite{experimentalConscious}, the authors stop the protocol heuristically. Hence, the count obtained is not guaranteed to be correct. Indeed, errors appear when the conductance of the underlying connectivity graph is low.
In our work, we aim for Counting algorithms that terminate returning always the correct count. 
The protocol in~\cite{oracle} is shown to eventually terminate, although the running time is not proved. In their model, it is assumed that each node is equipped with an oracle that provides an estimation of its degree at each round. This is still an assumption of knowledge of network characteristics, although local.
This and the above shortcomings are not unexpected in light of the conjecture in~\cite{spirakis}, which states that
Counting (actually, any non-trivial computations) in \ADNs
without knowledge of some network characteristics is impossible.
Nevertheless, a proof of such conjecture has not been found yet.

Known lower bounds for Counting in \ADNs include only the trivial $\Omega(D)$, where $D$ is the \emph{dynamic} diameter of the network, and $\Omega(\log n)$~\footnote{Throughout the paper, $\log$ means logarithm base $2$, unless otherwise stated.} even if $D$ is constant, proved in~\cite{baldoni}. 


